What Are You Token About? Dense Retrieval as Distributions Over the Vocabulary

Dual encoders are now the dominant architecture for dense retrieval. Yet, we have little understanding of how they represent text, and why this leads to good performance. In this work, we shed light on this question via distributions over the vocabulary. We propose to interpret the vector representations produced by dual encoders by projecting them into the model's vocabulary space. We show that the resulting projections contain rich semantic information, and draw connection between them and sparse retrieval. We find that this view can offer an explanation for some of the failure cases of dense retrievers. For example, we observe that the inability of models to handle tail entities is correlated with a tendency of the token distributions to forget some of the tokens of those entities. We leverage this insight and propose a simple way to enrich query and passage representations with lexical information at inference time, and show that this significantly improves performance compared to the original model in zero-shot settings, and specifically on the BEIR benchmark.

==> 05_analysis_results.tex <==

\section{Vocabulary Projections: Analysis}\label{sec:properties}

In Section~\ref{sec:framework}, we introduce a new framework for interpreting representations produced by dense retrievers.
Next, we describe empirical findings that shed new light on what is encoded in these representations. Via vocabulary projections, we draw connections between dense retrievers and well-known concepts like \textit{lexical overlap} and \textit{lexical expansion}. We start by analyzing query representations (\S\ref{sec:question-analysis}) and then move to the analysis of passages (\S\ref{sec:passage-analysis}).


% \input{fig_pie_charts.tex}
\input{fig_stacked_bar.tex}

\subsection{Projecting Query Representations}\label{sec:question-analysis}
\amir{title here should presumably be "Query Vocabulary Projections" which we mention in the intro. We need to be consistent about this.}
We begin our analysis by considering the top-scored items in vocabulary projections of queries. 
We ask: \textit{are these words present in the question and/or its gold passage?} Answering this question may help draw conclusions on how a dense retriever builds its representations. 
For example, we wish to investigate to what extent are \textit{lexical overlap} and \textit{query expansion}, which are fundamental concepts in sparse retrieval, encoded in query representations.
Consider the first example in Table~\ref{tab:examples}.  Two of the tokens shared by the question and passage (``\textcolor{applegreen}{lakes}'' and ``\textcolor{applegreen}{ocean}'') are among the top-ranked in $Q$, therefore they are viewed as the \textit{lexical overlap} signal. Also, six tokens from the passage \textit{not present in the question} (``\textcolor{blue}{river}'', ``\textcolor{blue}{north}'', ``\textcolor{blue}{canada}'', ``\textcolor{blue}{east}'', ``\textcolor{blue}{border}'', ``\textcolor{blue}{michigan}'') are also ranked high, thus we view them as \textit{query expansion}. We now turn to quantify these phenomena.

To that end, Figure~\ref{fig:q_pie_charts} analyzes the top-scored (\textit{i.e.}, top-$k$) tokens in $Q$, the vocabulary projections corresponding to the question. 
% Specifically, we take the questions, as well as their corresponding gold positive passages, in the development set of NQ. 
Specifically, for each question $q$ and its corresponding gold passage $p$ in the development set of NQ, we compute the question vocabulary projection $Q$, and report the overlap between top-$k$ tokens in $Q$, and
the tokens in $q$ and $p$. Overall, it is evident that the tokens of $q$ and $p$ constitute a major part of the top-scored tokens in $Q$ (the union of the blue, red and yellow slices), and the top-scored token (Figure~\ref{fig:q_pie_charts}a) is present in at least one of them in 87.2\% of the questions. This is evidence that these tokens are meaningful with respect to both $q$ and $p$.

\paragraph{Lexical Overlap} Tokens shared by $q$ and $p$ constitute the \textit{lexical overlap} signal in retrieval, used by sparse methods like BM25. \textit{How prominent are they in question projections?} Figure~\ref{fig:q_pie_charts} illustrates that for more than 70\% of the questions, the first token in $Q$ \textit{appears in both} the question $q$ and its gold passage $p$ (yellow slice). When considering the top-5 tokens in $Q$, more than 30\% of the tokens are shared tokens. 
These findings emphasize that even for dense retrievers---which do not operate at the lexical level---lexical overlap remains a highly dominant signal. 

\input{table_token_mrr_P.tex}
\paragraph{Query Expansion}  To overcome the ``vocabulary mismatch'' problem (\textit{i.e.}, when question-document pairs are semantically relevant, but lack significant lexical overlap), \textit{query expansion} methods have been studied extensively \cite{relevance-feedback,qexpansion1,qexpansion2,mao-etal-2021-generation}. The main idea is to expand the query with additional terms that will better guide the retrieval process. Figure~\ref{fig:q_pie_charts} suggests that query expansion is also dominant in dense retrieval. We define a token as a query expansion if it does not appear in the query itself but does appear in the query projection $Q$, and also in the gold passage of that query $p$. 
Surprisingly, almost 14\% of the tokens in the top-5 of $Q$ are query expansion tokens (red slices). We note that there are two interesting classes of query expansion tokens: (1) synonyms of question tokens, as well as tokens that share similar semantics with tokens in $q$ (\textit{e.g.}, ``\textcolor{blue}{michigan}'' in the first example of Table~\ref{tab:examples}). (2) ``answer tokens'' which contain the answer to the query (\textit{e.g.}, ``\textcolor{blue}{motown}'' in the second example of Table~\ref{tab:examples}). The presence  of such tokens may suggest the model already ``knows'' the answer to the given question, either from pretraining or from similar questions seen during training.

\subsection{Projecting Passage Representations}\label{sec:passage-analysis}

We continue our projection-based analysis of dense retrievers by asking, \textit{what is encoded in passage representations?} We show that vocabulary projections can provide intuitive explanations and discover interesting phenomena concerning this question as well. 

Encoding passages is a fundamentally different task than encoding questions, as the former contain significantly more information than the latter.\footnote{The average question length in Natural Questions (using BERT's vocabulary) is 9.8 tokens, while the average passage length in our corpus is 135 tokens.
} 
% Next, we delve deeper into how dense retrievers \ori{continue..}
Intuitively, a passage representation should focus on information that is likely to be asked about.  
We now investigate whether this intuition is manifested in passage vocabulary projections.
% Surprisingly, we show that this intuition is manifested in passage vocabulary projections -- tokens from the passage that are contained in likely questions, are ranked higher than others. In addition, we show that \textit{document expansion} (i.e., tokens that appear in relevant questions but not in the passage itself) is rare. \yb{again, I'd move the interpretation of the results to be after the results; here, I'd just pose the questions we're asking, then answer, then interpre}

\paragraph{Query Prediction} We start our passage-side analysis by hypothesizing that out of passage tokens, \textit{those that are likely to appear in relevant questions receive higher scores than others}. 
To test our hypothesis, we analyze the ranks of question and passage tokens in passage vocabulary projections, $P$. Formally, let $\mathcal{T}_q$ and $\mathcal{T}_p$ be the \textit{sets} of tokens in a question $q$ and its gold passage $p$, respectively.
Table~\ref{tab:token-mrr} exhibits the token-level mean reciprocal rank (MRR) of these sets in $P$. 
We observe that tokens shared by $q$ and $p$ (\textit{i.e.}, $\mathcal{T}_q\cap \mathcal{T}_p$) are ranked significantly higher than other passage tokens (\textit{i.e.}, $\mathcal{T}_p$). For example, in DPR the MRR of shared tokens is 0.26, while that of other passage tokens is only 0.03.
This trend holds for other models as well.
This finding thus supports our claim and quantifies that tokens that appear in relevant questions are ranked higher than others. 
This behavior suggests that the model \textit{predicts} which of the input passage tokens will appear in likely questions.

\input{fig_failure}

Additionally, the results in Table~\ref{tab:token-mrr} suggest an intuitive explanation to why unsupervised dense retrievers like Spider still lag behind supervised ones as DPR and S-MPNet (especially in top-$k$ accuracy for lower values of $k$, \textit{cf}. Spider results in Table~\ref{tab:nq-results}): unsupervised models are dramatically less effective in query prediction (\textit{e.g.}, the MRR of shared tokens in Spider is 0.12, compared to 0.26 and 0.25 in DPR and S-MPNet). 
This might be due to the fact that unsupervised models do not observe real questions in their training (\textit{e.g.}, Spider synthesizes pseudo-questions on real passages), and are thus less effective in query prediction.

\paragraph{(Lack of) Document Expansion} 
In \S\ref{sec:question-analysis}, we argue that dense models implicitly apply query expansion to drive their retrieval process. However, expanding documents (or passages) is also a popular approach for improving retrieval \cite{tao-etal-2006-language,pexpansion3,pexpansion1,pexpansion2}. \textit{Is document expansion used by dense retrievers?} We find signals suggesting this is \textit{not} the case. Table~\ref{tab:token-mrr} indicates that tokens from $\mathcal{T}_q\setminus\mathcal{T}_p$ (\textit{i.e.}, tokens that appear in $q$ but not in $p$) are not frequent among the top-scored tokens in $P$, as their MRR values is particularly low, 0.01--0.02. Also, Figure~\ref{fig:dpr_p_pie_charts} demonstrates that these tokens constitute only 1\% of the top-$k$ tokens in $P$ (blue slices). We hypothesize that since there are many questions that can be asked for a single passage, anticipating the relevant lexical expansion is challenging.






% Specifically, tokens shared by $q$ and $p$ that are scored high in both $Q$ and $P$ can be thought of as ``lexical overlap'' signal. Tokens that appear in the passage $p$ and not in $q$ -- but ranked high in $Q$ -- can be though of as ``query expansion'' \cite{relevance-feedback,mao-etal-2021-generation}. Similarly, tokens that appear in the question $q$ but not in $p$ -- and ranked high in $P$ -- can be though of as ``document expansion'' \cite{pexpansion1,pexpansion2}.
% Interestingly, in roughly 87\% of the questions the highest-ranked token ($k=1$) is found in the question and/or its gold positive passage. In 71\% of the questions, the token appears in both. An example is the top case in Figure~\ref{fig:intro_two_examples}, where the token ``court'' is found in both, and is ranked first in $Q$. This may suggest that lexical overlap is used as a strong signal by dense retrievers. When considering the top-5 tokens in the question, more than 50\% of the tokens appear either in $q$ or $p$. 
% \textit{Query expansion} (i.e., ``token only in passage'') accounts for almost 14\% of the tokens for $k=5$, \ori{Interpretation?}.

% Similar analysis for passage vocabulary projections $P$ is given in App.~\ref{app:token_analysis}. 
% Contrary to query expansion, document expansion tokens are significantly less frequent (roughly 1\% of the tokens for all $k$-s). 
% This finding may indicate that \ori{interpretation?}.


% \input{fig_kl_example}



==> fig_kl_example.tex <==
\begin{figure}[t]
\centering
% \hspace*{-20pt}
\includegraphics[width=\columnwidth]{figures/dpr_nq-dev_kl.pdf}
\vspace{-10pt}
\caption{An example of the correlation between distributional similarity in vocabulary space (measured by negative KL divergence) and model scores (dot product in representation space) for a random question from NQ, given by DPR. 
}
\label{fig:example_kl}
\end{figure}

==> fig_pie_charts.tex <==
\begin{figure}[t!]
\centering
\subfloat[$k=1$]{%
  \includegraphics[clip,width=\columnwidth]{figures/token_pie_dpr_nq-dev_k1.pdf}%
}

\subfloat[$k=5$]{%
\includegraphics[clip,width=\columnwidth]{figures/token_pie_dpr_nq-dev_k5.pdf}%
}

\subfloat[$k=20$]{%
\includegraphics[clip,width=\columnwidth]{figures/token_pie_dpr_nq-dev_k20.pdf}%
}
\caption{An analysis of the top-$k$ tokens in the vocabulary projection $Q$ of DPR on questions in the development set of NQ. Specifically, we analyze whether these tokens are present in the question and/or in its gold positive passage. Similar analysis for $P$ is given in Figure~\ref{fig:dpr_p_pie_charts}.
}\label{fig:q_pie_charts}
\end{figure}

==> fig_token_analysis_dpr_P.tex <==
\begin{figure}[t!]
\centering
\subfloat[$k=1$]{%
  \includegraphics[clip,width=\columnwidth]{figures/token_pie_dpr_nq-dev_P_k1.pdf}%
}

\subfloat[$k=5$]{%
\includegraphics[clip,width=\columnwidth]{figures/token_pie_dpr_nq-dev_P_k5.pdf}%
}

\subfloat[$k=20$]{%
\includegraphics[clip,width=\columnwidth]{figures/token_pie_dpr_nq-dev_P_k20.pdf}%
}
\caption{An analysis of the top-$k$ tokens in the vocabulary projection $P$ of DPR on gold passages of questions in the development set of NQ. Specifically, we analyze whether these tokens are present in the gold passage and/or in its corresponding question. Similar plots for $Q$ are given in Figure~\ref{fig:q_pie_charts}.
}\label{fig:dpr_p_pie_charts}
\end{figure}

==> table_models.tex <==

\begin{table*}[t]
\centering
\small
\begin{tabular}{lllll}
\toprule
\textbf{Model} & & \textbf{Training Dataset} & \textbf{Pretrained Model} & \textbf{Pooling} \\
\midrule
\multicolumn{5}{c}{\textit{Supervised Models}}  \\
\midrule
DPR & \citet{karpukhin-etal-2020-dense} & Natural Questions & BERT-base & CLS \\
S-MPNet & \citet{mpnet}  & Diverse & MPNet-base & Mean \\
% GTR-base & \citet{gtr}  & Community QA \& MS MARCO & T5-base & Mean \\
\midrule
\multicolumn{5}{c}{\textit{Unsupervised Models}}  \\
\midrule
Spider & \citet{ram-etal-2022-learning} & Wikipedia & BERT-base & CLS \\
SPAR ? & \citet{spar} & Wikipedia & BERT-base & CLS \\
\bottomrule
\end{tabular}
\caption{caption}
\label{table:models}
\end{table*}

==> table_nq_results.tex <==
\begin{table}[t!]
\small
\centering
\begin{tabular}{lcccc}
\toprule
\multirow{2.6}{55pt}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{NQ}}  \\
\cmidrule(lr){2-5}
& \textbf{Top-1} & \textbf{Top-5} & \textbf{Top-20} & \textbf{Top-100} \\
\midrule
DPR & \textbf{46.3} & \textbf{68.3} & 80.1 & 86.1 \\
DPR + LE & 45.8 & 67.8 & \textbf{80.8} & \textbf{87.2} \\
\midrule
S-MPNet & 37.7 & \textbf{66.4} & \textbf{80.9} & 87.8 \\
S-MPNet + LE & \textbf{39.3} & 66.0 & 80.2 & \textbf{88.0} \\
\midrule
Spider & 24.8 & 49.6 & \textbf{68.3} & 81.2 \\
Spider + LE & \textbf{25.9} & \textbf{50.4} & 67.8 & \textbf{81.4} \\
\bottomrule
\end{tabular}
\caption{Top-$k$ retrieval accuracy of different models on the test set of NQ,  with and without lexical enrichment (LE).
NQ was used for training DPR and S-MPNet.
}
\label{tab:nq-results}
\end{table}
